Real Time Incremental Foveal Texture Mapping for Autonomous Vehicles

We propose an end-to-end real time framework to generate high resolution graphics grade textured 3D map of urban environment. The generated detailed map finds its application in the precise localization and navigation of autonomous vehicles. It can also serve as a virtual test bed for various vision and planning algorithms as well as a background map in the computer games. In this paper, we focus on two important issues: (i) incrementally generating a map with coherent 3D surface, in real time and (ii) preserving the quality of color texture. To handle the above issues, firstly, we perform a pose-refinement procedure which leverages camera image information, Delaunay triangulation and existing scan matching techniques to produce high resolution 3D map from the sparse input LIDAR scan. This 3D map is then texturized and accumulated by using a novel technique of ray-filtering which handles occlusion and inconsistencies in pose-refinement. Further, inspired by human fovea, we introduce foveal-processing which significantly reduces the computation time and also assists ray-filtering to maintain consistency in color texture and coherency in 3D surface of the output map. Moreover, we also introduce texture error (TE) and mean texture mapping error (MTME), which provides quantitative measure of texturing and overall quality of the textured maps.

==> implementation.tex <==
\subsubsection{Map Representation}
A map can be of extremely large size (e.g. map of cities), therefore, any algorithm should be able to handle these maps in a manner such that memory and computational resources required are minimal. In this work we use a grid based representation of the 3D textured map. We divide the 3D map into 2D grids (tiles) where each tile stores its own point cloud. Typically such a 2D tile can be represented by 3 parameters tile length, tile width and starting coordinates.
%
%
% 
%Figure \ref{fig_grid} shows such a grid having four tiles. Arrow in the figure shows, grid continues to expand. Eq. \ref{eq_tile} represents a typical tile with starting coordinates $x,y$, length L, width W and height ranging from $-\inf~to~\inf$ .
%%
%%
%%
%\begin{equation}
%\begin{split}
%tile = ~x<X<x+L,\\~y<Y<Y+W,\\~-\inf<z<\inf
%\end{split}
%\label{eq_tile}
%\end{equation} 
%%
%%
%\begin{figure}
%\centering
%\includegraphics[height=0.9\linewidth, width=0.9\linewidth]{images/grid.jpg}
%\label{fig_grid}
%\caption{A Typical 2D Grid having four tiles}
%\end{figure}
%%
%%
%\indent\par
This representation of the point cloud allows us to visualize and process large 3D maps despite limited RAM in computers. The \textit{tiled} architecture allows us to load the point cloud corresponding to the region of interest. Moreover, while processing the point cloud in the map, only a local region is required, hence there is no need to load complete point cloud in the memory even at the processing time. However, for the boundary points corresponding to each tile, points from neighboring tiles are also required to be taken into account.
% \indent\par
% Further, each tile is processed separately, lets say it \textit{target tile}. Since it might happen that a tile is continuous at the boundaries i.e. part of 3D object lies in one tile and part in other tiles. So to process a tile, points from the neighboring tiles have to be taken into account.
%%
%%
%\begin{figure}[h]
%\centering
%\includegraphics[height=0.9\linewidth, width=0.9\linewidth]{images/nbr_tiles.jpg}
%\label{fig_nbr_tiles}
%\caption{An illustration of target and neighboring tiles concept}
%\end{figure}
%%
%%
%%
%Fig \ref{fig_nbr_tiles} shows a target tile and its neighbors.
%
For instance, for estimating normals for the boundary points, some part of the local continuous surface may be lying in the neighboring tiles. If we consider this tile architecture, a maximum of 8 neighboring tiles are required in order to process all the points in a given $target~tile$.


























